Robust Gaussian Covariance Estimation in Nearly-Matrix Multiplication Time

Robust covariance estimation is the following, well-studied problem in high dimensional statistics: given $N$ samples from a $d$-dimensional Gaussian $\mathcal{N}(\boldsymbol{0}, \Sigma)$, but where an $\varepsilon$-fraction of the samples have been arbitrarily corrupted, output $\widehat{\Sigma}$ minimizing the total variation distance between $\mathcal{N}(\boldsymbol{0}, \Sigma)$ and $\mathcal{N}(\boldsymbol{0}, \widehat{\Sigma})$. This corresponds to learning $\Sigma$ in a natural affine-invariant variant of the Frobenius norm known as the \emph{Mahalanobis norm}. Previous work of Cheng et al demonstrated an algorithm that, given $N = \Omega (d^2 / \varepsilon^2)$ samples, achieved a near-optimal error of $O(\varepsilon \log 1 / \varepsilon)$, and moreover, their algorithm ran in time $\widetilde{O}(T(N, d) \log \kappa / \mathrm{poly} (\varepsilon))$, where $T(N, d)$ is the time it takes to multiply a $d \times N$ matrix by its transpose, and $\kappa$ is the condition number of $\Sigma$. When $\varepsilon$ is relatively small, their polynomial dependence on $1/\varepsilon$ in the runtime is prohibitively large. In this paper, we demonstrate a novel algorithm that achieves the same statistical guarantees, but which runs in time $\widetilde{O} (T(N, d) \log \kappa)$. In particular, our runtime has no dependence on $\varepsilon$. When $\Sigma$ is reasonably conditioned, our runtime matches that of the fastest algorithm for covariance estimation without outliers, up to poly-logarithmic factors, showing that we can get robustness essentially "for free."

==> SE-mean-estimation.tex <==
\section{Robust Covariance Estimation}
\subsection{Reduction From Robust Covariance Estimation to Robust Mean Estimation}
There is a well-known trick to reduce the problem from unknown mean, unknown covariance, to zero mean unknown covariance; for example see  4.5.1 of \cite{DBLP:conf/focs/DiakonikolasKK016}.  Now, we can assume the distribution $D$ is zero mean. 
Note that, when $X$ is a zero mean random variable, we have $\-E[XX^\top] = \Sigma$, then we can reduce the robust covariance estimation problem to covariance mean estimation.  Let $Z_i = X_i \otimes X_i$. Since $X_i$'s are subgaussian random variables, then we know that $Z_i$'s are subexponential random variables, for example see \cite{DBLP:conf/aistats/HonorioJ14}.
For the covariance of $Z$, we have the following lemma:
\begin{lemma}[Lemma 2.1 of \cite{DBLP:conf/colt/0002D0W19}]
Let $X\sim D$ where $D$ is a Gaussian distribution with mean $0$ and covariance $\Sigma$ and $Z=X\otimes X$. Let $\Sigma_Z \in R^{d^2\times d^2}$ be the covariance matrix of $Z$. We have: \\
1. If $\Sigma \preceq I$, then $\Sigma_Z \preceq 2I$. \\
2. If $0\leq \tau < 1$ and $\|\Sigma-I\|_2 \leq \tau$, then $\|\Sigma_Z -2I\|_2 \leq 6\tau$.
\end{lemma}

\subsection{Subexponential Random Variables are Subgaussian Good}
\begin{definition}[Subgaussian goodness in \cite{DBLP:journals/corr/abs-1906-11366}]
\label{def:sg-goodness}
Let $D$ be a distribution with covariance $\Id$ and mean $\mu$.
We say a set of points $S$ is \emph{$(\eps, \gamma_1, \gamma_2, \beta_1, \beta_2)$-subgaussian good} (or $(\eps, \gamma_1, \gamma_2, \beta_1, \beta_2)$-s.g. good for short) with respect to $D$ if  the following inequalities are satisfied:
\begin{itemize}
\item $\Norm{\mu(S) - \mu} \leq \gamma_1$ and $\Norm{\frac{1}{|S|} \sum_{i \in S} \Paren{X_i - \mu(S)} \Paren{X_i - \mu(S)}^\top - \Id}_2 \leq \gamma_2$, and
\item For any subset $T \subset S$ so that $|T| = 2 \eps |S|$, we have
\begin{align*}
\Norm{\frac{1}{|T|} \sum_{i \in T} X_i - \mu} \leq \beta_1 \; ,~\mbox{and}~ \Norm{\frac{1}{|T|} \sum_{i \in T} \Paren{X_i - \mu(S)} \Paren{X_i - \mu(S)}^\top - \Id}_2 \leq \beta_2 \; .
\end{align*}
\end{itemize}
\end{definition}
\noindent
For conciseness, when the parameters $\eps, \gamma_1, \gamma_2, \beta_1, \beta_2$ are understood, we will omit them and refer to the data set as s.g.-good.


In \cite{DBLP:journals/corr/abs-1906-11366}, they showed that for any distribution satisfies the subgaussian goodness in \cref{def:sg-goodness}, then there exists an efficient algorithm for robust mean estimation:
\begin{theorem}\label{thm:sg-algo}
Let $D$ be a distribution on $\R^d$ with mean $\mu$ and variance proxy $1$. Let $\eps < c$, where $c$ is a universal constant, let $\gamma_1,\gamma_2.\beta_1,\beta_2 >0$. Let $S$ be a dataset, $|S| = n$, so that $S = S_g \cap S_b\setminus S_r$ so that $S_g$ is $(\eps,\gamma_1,\gamma_2.\beta_1,\beta_2)$-s.g. good with respect to $D$, and $|S_b|,|S_r| \leq \eps|S|$. Then, there exists an algorithm \textsc{s.g.-QUEScoreFilter($S, \eps, \cO_{\mathrm{approx}}$)} outputs a $\hat{\mu}$ so that
\[
\| \hat{\mu} - \mu \|_2 \leq O \Paren{\gamma_1 + \eps \sqrt{\log 1 / \eps} + \sqrt{\eps \xi }} \; ,
\]
where 
\begin{equation}
\label{eq:xi-def}
\xi = \xi (\eps, \gamma_1, \gamma_2, \beta_1, \beta_2) = \gamma_2 + 2 \gamma_1^2 + 4 \eps^2 \beta_1^2 + 2 \eps \beta_2 + O(\eps \log 1 / \eps) \; .
\end{equation}
Moreover, this algorithm requires $O(\log d)$ calls to $\cO_{\mathrm{approx}}$, and requires $\widetilde{O}(nd)$ additional computation.

\end{theorem}

It turns out, the subexponential distribution also satisfies the s.g.\ goodness with slightly worse parameters:
\begin{lemma}
\label{lem:conc-SE}
Let $Z_1, \ldots, Z_n \sim D$ and $Z_i \in \R^{d^2}$, where $D$ is subexponential with variance proxy $1$.
Then, for any $\eps > 0$ sufficiently small, we have that $S = \{X_1, \ldots, X_n\}$ is $\Paren{\eps, \gamma_1, \gamma_2 }$-s.g. good with probability $1 - \delta$, where
\begin{align}
\gamma_1 = O \Paren{ \max \Paren{ \sqrt{\frac{d^2 + \log 1 / \delta}{n}}, \frac{d^2 + \log 1 / \delta}{n}}}  \; &,~\gamma_2 = O \Paren{ \max \Paren{ {\frac{d^2 + \log 1 / \delta}{n}}, \Paren{\frac{d^2 + \log 1 / \delta}{n}}^2}} \; , \mbox{and} \label{eq:conc-SE} \\
\beta_1 = O \Paren{\log 1 / \eps + \frac{d^2 + \log 1 / \delta}{\eps n}} \; ,~&\mbox{and}~ \beta_2 = O \Paren{\log^2 1 / \eps + \Paren{\frac{d^2 + \log 1 / \delta}{\eps n}}^2} \; . \label{eq:conc-SE-2}
\end{align}
\end{lemma}
Then, in particular, note that when $n = \Omega\Paren{\frac{d^2+\log 1/\delta}{\eps^2 \log 1/\eps}}$, then the \cref{lem:conc-SE} implies $n$ i.i.d. samples from an isotropic subexponential distribution is $(\eps, O(\eps\log 1/\eps), O((\eps\log1/\eps)^2), O(\log 1/\eps), O((\log 1/\eps)^2))$-s.g. good with probability $1-\delta$. This implies we can find some $\hat{\mu}$ such that 
\[
\| \hat{\mu} - \mu \|_2 \leq O \Paren{\eps \log 1/\eps} \; .
\]



To prove \cref{lem:conc-SE}, we will require the following tail bound for the subexponential random variable
\begin{lemma}\label{lem:SE-tail}
Let $Z_1, \ldots, Z_n \sim D$ and $Z_i \in \R^{d^2}$, where $D$ is is a subexponential distribution with mean $0$ and covariance $\Sigma \preceq I$. Let $v\in \R^{d^2}$ be an arbitrary unit vector. Then, there exists a universal constant $B>0$ such that for all $T> 0$ , we have 
\begin{align*}
    \Pr\left[\abs{\frac{1}{n} \sum_{i=1}^n \langle v, Z_i \rangle } > T\right] \leq 2\exp(-B n \min(T^2, {T})).
\end{align*}
\end{lemma}

To control the tail bound of square of subexponential random variable, we have the following concentration inequality.
\begin{lemma}[Proposition 1.1 of \cite{1903.05964}]\label{lem:SE-hanson-wright}
Let $Z_1, \ldots, Z_n \sim D$ and $Z_i \in \R^{d^2}$, where $D$ is a subexponential distribution with mean $0$ and covariance $\Sigma \preceq I$. Let $U \in \R^{d\times d}$ satisfy $U \succeq 0$ and $\|U\|_F = 1$. Then, there exists a universal constant $B > 0$ so that for all $T > 0$, we have 
\begin{align*}
    \Pr\left[\abs{\frac{1}{n} \sum_{i=1}^n \tr(Z_iZ_i^\top U) - \tr(U)} > T\right] \leq 2\exp(-B n \min(T^2, \sqrt{T})).
\end{align*}
\end{lemma}

By a standard $\eps$-net argument, for example see \cite{DBLP:journals/corr/abs-1011-3027}, we have the following concentration bound
\begin{lemma}\label{lem:SE-l2norm}
Let $Z_1, \ldots, Z_n \sim D$ and $Z_i \in \R^{d^2}$, where $D$ is a subexponential distribution with mean $0$ and covariance $\Sigma \preceq I$. Then, there exists a universal constant $A,B>0$ such that for all $T> 0$ , we have 
\begin{align*}
    \Pr\left[\Norm{\frac{1}{n} \sum_{i=1}^n Z_i}_2 > T\right] \leq 2\exp(Ad^2-B n \min(T^2, {T})).
\end{align*}
\end{lemma}
\begin{lemma}\label{lem:SE-covariance}
Let $Z_1, \ldots, Z_n \sim D$ and $Z_i \in \R^{d^2}$, where $D$ is a subexponential distribution with mean $0$ and covariance $\Sigma \preceq I$. Then, there exists a universal constant $A,B>0$ such that for all $T> 0$ , we have 
\begin{align*}
    \Pr\left[\Norm{\frac{1}{n} \sum_{i=1}^n Z_iZ_i^\top -I}_2 > T\right] \leq 2\exp(Ad^2-B n \min(T^2, \sqrt{T})).
\end{align*}
\end{lemma}
\begin{proof}[Proof of \cref{lem:conc-SE}]
For \cref{eq:conc-SE}, it suffices to directly use concentration bound of \cref{lem:SE-l2norm,lem:SE-covariance}. For the \cref{eq:conc-SE-2}, we can obtain the result by taking a union bound of all sets of size $\eps n$.
\end{proof}


\subsection{Iterative Refinement}
To use \cref{thm:sg-algo}, it requires the distribution $D$ has covariance bounded by $I_d$. Then, we need find a good start point before we can use such algorithm:
\begin{lemma}[Lemma 3.1 of \cite{DBLP:conf/colt/0002D0W19}]
We can compute a matrix $\Sigma_0$ in $\widetilde{O}(Nd^{1.26})$ time such that, with high probability, $\Sigma \preceq \Sigma_0 \preceq (\kappa\operatorname{poly}(d))\Sigma$ and $\Sigma_0 \leq \operatorname{poly}(d) \|\Sigma\|_2$.
\end{lemma}

Then, let $Y_i = \Sigma_0^{-1/2}X_i$ and $Z_i =\frac{1}{\sqrt{2}} Y_i\otimes Y_i$. Then, when $X_i \sim \+N(0, \Sigma)$, the covariance matrix of $Y$ is $\Sigma_Y = \Sigma_0^{-1/2}\Sigma \Sigma_0^{-1/2} \preceq I$, so the mean of $Z$ is $\-E[Z] = \frac{1}{\sqrt{2}}(\Sigma_0^{-1/2}\Sigma \Sigma_0^{-1/2})^\flat$. Then, by \cref{lem:SE-covariance}, we have the covariance matrix of $\Sigma_Z \preceq I$. Then, let $M$ be the output of \textsc{s.g.-QUEScoreFilter($Z_1,\ldots, Z_n$)}. Then, we have guarantee that 
\begin{align*}
    \Norm{\sqrt{2}M-\Sigma_0^{-1/2}\Sigma \Sigma_0^{-1/2}}_F \leq O(\eps \log 1/\eps).
\end{align*}
Let $\widehat{\Sigma} = \Sigma_0^{1/2} (\sqrt{2}M) \Sigma_0^{1/2}$, we have 
\begin{align*}
    \Norm{\widehat{\Sigma}-\Sigma}_F = \Norm{\Sigma_0^{1/2} (\sqrt{2}M) \Sigma_0^{1/2} - \Sigma} \leq O(\eps \log 1/\eps).
\end{align*}



